Learning Clique Forests

We propose a topological learning algorithm for the estimation of the conditional dependency structure of large sets of random variables from sparse and noisy data. The algorithm, named Maximally Filtered Clique Forest (MFCF), produces a clique forest and an associated Markov Random Field (MRF) by generalising Prim's minimum spanning tree algorithm. To the best of our knowledge, the MFCF presents three elements of novelty with respect to existing structure learning approaches. The first is the repeated application of a local topological move, the clique expansion, that preserves the decomposability of the underlying graph. Through this move the decomposability and calculation of scores is performed incrementally at the variable (rather than edge) level, and this provides better computational performance and an intuitive application of multivariate statistical tests. The second is the capability to accommodate a variety of score functions and, while this paper is focused on multivariate normal distributions, it can be directly generalised to different types of statistics. Finally, the third is the variable range of allowed clique sizes which is an adjustable topological constraint that acts as a topological penalizer providing a way to tackle sparsity at $l_0$ semi-norm level; this allows a clean decoupling of structure learning and parameter estimation. The MFCF produces a representation of the clique forest, together with a perfect ordering of the cliques and a perfect elimination ordering for the vertices. As an example we propose an application to covariance selection models and we show that the MCFC outperforms the Graphical Lasso for a number of classes of matrices.

==> Tables/Chordal.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:07:09 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rlrrrrrrr}
  \hline
Series length & Algorithm & Mean Log-likelihood & Stdev Log-likelihood & Mean number of parameters in inverse & Min clique size & Median clique size & Max clique size & Penalty/Shrinkage parameter \\ 
  \hline
 25 & GLASSO\_XVAL & -2882.80 & 695.86 & 1194.00 &  &  &  & 0.15 \\ 
   25 & MFCF\_FIX & -799.43 & 1537.30 & 99.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   25 & MFCF\_FIX\_ID & -817.47 & 1529.44 & 99.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   25 & MFCF\_VAR & -793.26 & 1544.70 & 98.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   25 & MFCF\_VAR\_ID & -811.31 & 1536.78 & 98.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   25 & REAL\_OR\_ML & 701.03 & 1512.24 & 164.00 &  &  &  &  \\ 
   25 & SHRINKAGE & -4200.59 & 267.92 & 4950.00 &  &  &  & 0.73 \\ 
   50 & GLASSO\_XVAL & -2232.17 & 664.71 & 1118.00 &  &  &  & 0.12 \\ 
   50 & MFCF\_FIX & 241.89 & 1459.22 & 99.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   50 & MFCF\_FIX\_ID & 238.47 & 1461.56 & 99.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   50 & MFCF\_VAR & 229.19 & 1553.42 & 135.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   50 & MFCF\_VAR\_ID & 229.28 & 1552.68 & 135.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   50 & REAL\_OR\_ML & 768.55 & 1500.74 & 164.00 &  &  &  &  \\ 
   50 & SHRINKAGE & -3590.65 & 558.26 & 4950.00 &  &  &  & 0.52 \\ 
   75 & GLASSO\_XVAL & -1804.68 & 1131.89 & 1161.00 &  &  &  & 0.10 \\ 
   75 & MFCF\_FIX & 400.90 & 1485.95 & 138.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   75 & MFCF\_FIX\_ID & 400.83 & 1487.15 & 138.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   75 & MFCF\_VAR & 410.29 & 1495.66 & 136.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   75 & MFCF\_VAR\_ID & 410.23 & 1496.80 & 136.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   75 & REAL\_OR\_ML & 696.69 & 1505.40 & 164.00 &  &  &  &  \\ 
   75 & SHRINKAGE & -3117.99 & 618.66 & 4950.00 &  &  &  & 0.37 \\ 
  100 & GLASSO\_XVAL & -1231.09 & 1363.62 & 1730.00 &  &  &  & 0.06 \\ 
  100 & MFCF\_FIX & 468.27 & 1506.67 & 158.00 & 2.00 &   3 & 3.00 & 0.00 \\ 
  100 & MFCF\_FIX\_ID & 468.24 & 1508.14 & 158.00 & 2.00 &   3 & 3.00 & 0.00 \\ 
  100 & MFCF\_VAR & 472.50 & 1515.53 & 191.00 & 2.00 &   3 & 4.00 & 0.00 \\ 
  100 & MFCF\_VAR\_ID & 472.18 & 1516.67 & 191.00 & 2.00 &   3 & 4.00 & 0.00 \\ 
  100 & REAL\_OR\_ML & 690.84 & 1528.89 & 164.00 &  &  &  &  \\ 
  100 & SHRINKAGE & -2643.30 & 888.05 & 4950.00 &  &  &  & 0.26 \\ 
  200 & GLASSO\_XVAL & -436.25 & 1399.52 & 2586.00 &  &  &  & 0.01 \\ 
  200 & MFCF\_FIX & 548.88 & 1521.87 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  200 & MFCF\_FIX\_ID & 548.13 & 1520.87 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  200 & MFCF\_VAR & 547.93 & 1518.79 & 195.00 & 2.00 &   3 & 4.00 & 0.00 \\ 
  200 & MFCF\_VAR\_ID & 546.42 & 1518.51 & 176.00 & 2.00 &   3 & 3.00 & 0.00 \\ 
  200 & REAL\_OR\_ML & 659.23 & 1524.31 & 164.00 &  &  &  &  \\ 
  200 & SHRINKAGE & -1277.56 & 1549.93 & 4950.00 &  &  &  & 0.07 \\ 
  300 & GLASSO\_XVAL & -145.02 & 1416.97 & 2632.00 &  &  &  & 0.01 \\ 
  300 & MFCF\_FIX & 594.35 & 1550.10 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  300 & MFCF\_FIX\_ID & 595.46 & 1552.54 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  300 & MFCF\_VAR & 596.03 & 1549.64 & 231.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  300 & MFCF\_VAR\_ID & 597.04 & 1551.98 & 231.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  300 & REAL\_OR\_ML & 662.61 & 1551.28 & 164.00 &  &  &  &  \\ 
  300 & SHRINKAGE & -566.08 & 1513.87 & 4950.00 &  &  &  & 0.02 \\ 
  400 & GLASSO\_XVAL & -34.19 & 1357.51 & 2549.00 &  &  &  & 0.01 \\ 
  400 & MFCF\_FIX & 598.96 & 1499.06 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  400 & MFCF\_FIX\_ID & 599.91 & 1501.13 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  400 & MFCF\_VAR & 601.84 & 1498.60 & 231.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  400 & MFCF\_VAR\_ID & 602.07 & 1498.56 & 231.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  400 & REAL\_OR\_ML & 653.18 & 1498.30 & 164.00 &  &  &  &  \\ 
  400 & SHRINKAGE & -295.88 & 1438.08 & 4950.00 &  &  &  & 0.02 \\ 
  500 & GLASSO\_XVAL & -3.83 & 1365.87 & 2451.00 &  &  &  & 0.01 \\ 
  500 & MFCF\_FIX & 580.88 & 1509.78 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  500 & MFCF\_FIX\_ID & 580.91 & 1510.12 & 236.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  500 & MFCF\_VAR & 582.46 & 1508.96 & 213.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  500 & MFCF\_VAR\_ID & 582.45 & 1509.28 & 231.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  500 & REAL\_OR\_ML & 620.99 & 1509.15 & 164.00 &  &  &  &  \\ 
  500 & SHRINKAGE & -69.26 & 1515.00 & 4950.00 &  &  &  & 0.00 \\ 
  750 & GLASSO\_XVAL & 66.79 & 1336.97 & 2254.00 &  &  &  & 0.01 \\ 
  750 & MFCF\_FIX & 587.58 & 1502.31 & 255.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  750 & MFCF\_FIX\_ID & 587.52 & 1502.28 & 255.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  750 & MFCF\_VAR & 586.60 & 1500.99 & 246.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  750 & MFCF\_VAR\_ID & 586.60 & 1500.99 & 246.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  750 & REAL\_OR\_ML & 615.98 & 1503.91 & 164.00 &  &  &  &  \\ 
  750 & SHRINKAGE & 204.10 & 1504.61 & 4950.00 &  &  &  & 0.00 \\ 
  1000 & GLASSO\_XVAL & 100.79 & 1336.30 & 2108.00 &  &  &  & 0.01 \\ 
  1000 & MFCF\_FIX & 590.33 & 1512.25 & 255.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  1000 & MFCF\_FIX\_ID & 590.33 & 1512.25 & 255.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  1000 & MFCF\_VAR & 537.03 & 1521.70 & 244.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  1000 & MFCF\_VAR\_ID & 537.03 & 1521.70 & 244.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  1000 & REAL\_OR\_ML & 612.48 & 1509.57 & 164.00 &  &  &  &  \\ 
  1000 & SHRINKAGE & 327.54 & 1518.19 & 4950.00 &  &  &  & 0.00 \\ 
  1500 & GLASSO\_XVAL & 130.50 & 1323.45 & 1867.00 &  &  &  & 0.01 \\ 
  1500 & MFCF\_FIX & 596.72 & 1498.24 & 294.00 & 3.00 &   4 & 5.00 & 0.00 \\ 
  1500 & MFCF\_FIX\_ID & 596.72 & 1498.24 & 294.00 & 3.00 &   4 & 5.00 & 0.00 \\ 
  1500 & MFCF\_VAR & 598.33 & 1499.63 & 281.00 & 3.00 &   4 & 5.00 & 0.00 \\ 
  1500 & MFCF\_VAR\_ID & 598.33 & 1499.63 & 281.00 & 3.00 &   4 & 5.00 & 0.00 \\ 
  1500 & REAL\_OR\_ML & 612.41 & 1499.87 & 164.00 &  &  &  &  \\ 
  1500 & SHRINKAGE & 431.36 & 1497.59 & 4950.00 &  &  &  & 0.00 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Likelihood of the models. Mean values over 5 distinct training / validation sets and for 10 test set each.} 
\label{tab:Chordal:1}
\end{table}


==> Tables/Chordal_acc.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:07:09 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rlrrrrrrr}
  \hline
Series length & Algorithm & Mean Log-likelihood & Stdev Log-likelihood & Mean number of parameters in inverse & Min clique size & Median clique size & Max clique size & Penalty/Shrinkage parameter \\ 
  \hline
 25 & GLASSO\_XVAL & -2882.80 & 695.86 & 1194.00 &  &  &  & 0.15 \\ 
   25 & MFCF\_FIX & -799.43 & 1537.30 & 99.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   25 & MFCF\_FIX\_ID & -817.47 & 1529.44 & 99.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   25 & MFCF\_VAR & -793.26 & 1544.70 & 98.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   25 & MFCF\_VAR\_ID & -811.31 & 1536.78 & 98.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   25 & REAL\_OR\_ML & 701.03 & 1512.24 & 164.00 &  &  &  &  \\ 
   25 & SHRINKAGE & -4200.59 & 267.92 & 4950.00 &  &  &  & 0.73 \\ 
   50 & GLASSO\_XVAL & -2232.17 & 664.71 & 1118.00 &  &  &  & 0.12 \\ 
   50 & MFCF\_FIX & 241.89 & 1459.22 & 99.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   50 & MFCF\_FIX\_ID & 238.47 & 1461.56 & 99.00 & 2.00 &   2 & 2.00 & 0.00 \\ 
   50 & MFCF\_VAR & 229.19 & 1553.42 & 135.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   50 & MFCF\_VAR\_ID & 229.28 & 1552.68 & 135.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   50 & REAL\_OR\_ML & 768.55 & 1500.74 & 164.00 &  &  &  &  \\ 
   50 & SHRINKAGE & -3590.65 & 558.26 & 4950.00 &  &  &  & 0.52 \\ 
   75 & GLASSO\_XVAL & -1804.68 & 1131.89 & 1161.00 &  &  &  & 0.10 \\ 
   75 & MFCF\_FIX & 400.90 & 1485.95 & 138.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   75 & MFCF\_FIX\_ID & 400.83 & 1487.15 & 138.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   75 & MFCF\_VAR & 410.29 & 1495.66 & 136.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   75 & MFCF\_VAR\_ID & 410.23 & 1496.80 & 136.00 & 2.00 &   2 & 3.00 & 0.00 \\ 
   75 & REAL\_OR\_ML & 696.69 & 1505.40 & 164.00 &  &  &  &  \\ 
   75 & SHRINKAGE & -3117.99 & 618.66 & 4950.00 &  &  &  & 0.37 \\ 
  100 & GLASSO\_XVAL & -1231.09 & 1363.62 & 1730.00 &  &  &  & 0.06 \\ 
  100 & MFCF\_FIX & 468.27 & 1506.67 & 158.00 & 2.00 &   3 & 3.00 & 0.00 \\ 
  100 & MFCF\_FIX\_ID & 468.24 & 1508.14 & 158.00 & 2.00 &   3 & 3.00 & 0.00 \\ 
  100 & MFCF\_VAR & 472.50 & 1515.53 & 191.00 & 2.00 &   3 & 4.00 & 0.00 \\ 
  100 & MFCF\_VAR\_ID & 472.18 & 1516.67 & 191.00 & 2.00 &   3 & 4.00 & 0.00 \\ 
  100 & REAL\_OR\_ML & 690.84 & 1528.89 & 164.00 &  &  &  &  \\ 
  100 & SHRINKAGE & -2643.30 & 888.05 & 4950.00 &  &  &  & 0.26 \\ 
  200 & GLASSO\_XVAL & -436.25 & 1399.52 & 2586.00 &  &  &  & 0.01 \\ 
  200 & MFCF\_FIX & 548.88 & 1521.87 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  200 & MFCF\_FIX\_ID & 548.13 & 1520.87 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  200 & MFCF\_VAR & 547.93 & 1518.79 & 195.00 & 2.00 &   3 & 4.00 & 0.00 \\ 
  200 & MFCF\_VAR\_ID & 546.42 & 1518.51 & 176.00 & 2.00 &   3 & 3.00 & 0.00 \\ 
  200 & REAL\_OR\_ML & 659.23 & 1524.31 & 164.00 &  &  &  &  \\ 
  200 & SHRINKAGE & -1277.56 & 1549.93 & 4950.00 &  &  &  & 0.07 \\ 
  300 & GLASSO\_XVAL & -145.02 & 1416.97 & 2632.00 &  &  &  & 0.01 \\ 
  300 & MFCF\_FIX & 594.35 & 1550.10 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  300 & MFCF\_FIX\_ID & 595.46 & 1552.54 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  300 & MFCF\_VAR & 596.03 & 1549.64 & 231.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  300 & MFCF\_VAR\_ID & 597.04 & 1551.98 & 231.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  300 & REAL\_OR\_ML & 662.61 & 1551.28 & 164.00 &  &  &  &  \\ 
  300 & SHRINKAGE & -566.08 & 1513.87 & 4950.00 &  &  &  & 0.02 \\ 
  400 & GLASSO\_XVAL & -34.19 & 1357.51 & 2549.00 &  &  &  & 0.01 \\ 
  400 & MFCF\_FIX & 598.96 & 1499.06 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  400 & MFCF\_FIX\_ID & 599.91 & 1501.13 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  400 & MFCF\_VAR & 601.84 & 1498.60 & 231.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  400 & MFCF\_VAR\_ID & 602.07 & 1498.56 & 231.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  400 & REAL\_OR\_ML & 653.18 & 1498.30 & 164.00 &  &  &  &  \\ 
  400 & SHRINKAGE & -295.88 & 1438.08 & 4950.00 &  &  &  & 0.02 \\ 
  500 & GLASSO\_XVAL & -3.83 & 1365.87 & 2451.00 &  &  &  & 0.01 \\ 
  500 & MFCF\_FIX & 580.88 & 1509.78 & 216.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  500 & MFCF\_FIX\_ID & 580.91 & 1510.12 & 236.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  500 & MFCF\_VAR & 582.46 & 1508.96 & 213.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  500 & MFCF\_VAR\_ID & 582.45 & 1509.28 & 231.00 & 3.00 &   3 & 4.00 & 0.00 \\ 
  500 & REAL\_OR\_ML & 620.99 & 1509.15 & 164.00 &  &  &  &  \\ 
  500 & SHRINKAGE & -69.26 & 1515.00 & 4950.00 &  &  &  & 0.00 \\ 
  750 & GLASSO\_XVAL & 66.79 & 1336.97 & 2254.00 &  &  &  & 0.01 \\ 
  750 & MFCF\_FIX & 587.58 & 1502.31 & 255.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  750 & MFCF\_FIX\_ID & 587.52 & 1502.28 & 255.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  750 & MFCF\_VAR & 586.60 & 1500.99 & 246.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  750 & MFCF\_VAR\_ID & 586.60 & 1500.99 & 246.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  750 & REAL\_OR\_ML & 615.98 & 1503.91 & 164.00 &  &  &  &  \\ 
  750 & SHRINKAGE & 204.10 & 1504.61 & 4950.00 &  &  &  & 0.00 \\ 
  1000 & GLASSO\_XVAL & 100.79 & 1336.30 & 2108.00 &  &  &  & 0.01 \\ 
  1000 & MFCF\_FIX & 590.33 & 1512.25 & 255.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  1000 & MFCF\_FIX\_ID & 590.33 & 1512.25 & 255.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  1000 & MFCF\_VAR & 537.03 & 1521.70 & 244.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  1000 & MFCF\_VAR\_ID & 537.03 & 1521.70 & 244.00 & 3.00 &   4 & 4.00 & 0.00 \\ 
  1000 & REAL\_OR\_ML & 612.48 & 1509.57 & 164.00 &  &  &  &  \\ 
  1000 & SHRINKAGE & 327.54 & 1518.19 & 4950.00 &  &  &  & 0.00 \\ 
  1500 & GLASSO\_XVAL & 130.50 & 1323.45 & 1867.00 &  &  &  & 0.01 \\ 
  1500 & MFCF\_FIX & 596.72 & 1498.24 & 294.00 & 3.00 &   4 & 5.00 & 0.00 \\ 
  1500 & MFCF\_FIX\_ID & 596.72 & 1498.24 & 294.00 & 3.00 &   4 & 5.00 & 0.00 \\ 
  1500 & MFCF\_VAR & 598.33 & 1499.63 & 281.00 & 3.00 &   4 & 5.00 & 0.00 \\ 
  1500 & MFCF\_VAR\_ID & 598.33 & 1499.63 & 281.00 & 3.00 &   4 & 5.00 & 0.00 \\ 
  1500 & REAL\_OR\_ML & 612.41 & 1499.87 & 164.00 &  &  &  &  \\ 
  1500 & SHRINKAGE & 431.36 & 1497.59 & 4950.00 &  &  &  & 0.00 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Performance of the models on a random clique forest. Mean values over 10 sample runs.} 
\label{tab:Chordal:2}
\end{table}


==> Tables/Chordal_paramno.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:07:17 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{|r|R{2cm}|R{2cm}|R{2cm}|R{2cm}|R{2cm}|R{2cm}|}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & SHRINKAGE \\ 
  \hline
25 & 1194 & 99 & 99 & 98 & 98 & 4950 \\ 
  50 & 1118 & 99 & 99 & 135 & 135 & 4950 \\ 
  75 & 1161 & 138 & 138 & 136 & 136 & 4950 \\ 
  100 & 1730 & 158 & 158 & 191 & 191 & 4950 \\ 
  200 & 2586 & 216 & 216 & 195 & 176 & 4950 \\ 
  300 & 2632 & 216 & 216 & 231 & 231 & 4950 \\ 
  400 & 2549 & 216 & 216 & 231 & 231 & 4950 \\ 
  500 & 2451 & 216 & 236 & 213 & 231 & 4950 \\ 
  750 & 2254 & 255 & 255 & 246 & 246 & 4950 \\ 
  1000 & 2108 & 255 & 255 & 244 & 244 & 4950 \\ 
  1500 & 1867 & 294 & 294 & 281 & 281 & 4950 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Mean number of non-zero coefficient in the precision matrix by length of time series} 
\label{tab:Chordal:param_no}
\end{table}


==> Tables/Chordal_shrink.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:07:16 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{|r|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & SHRINKAGE \\ 
  \hline
  25 & 0.150 & 0.005 & 0.005 & 0.005 & 0.005 & 0.726 \\ 
    50 & 0.120 & 0.002 & 0.002 & 0.002 & 0.001 & 0.522 \\ 
    75 & 0.102 & 0.002 & 0.001 & 0.002 & 0.001 & 0.374 \\ 
   100 & 0.056 & 0.001 & 0.001 & 0.001 & 0.001 & 0.257 \\ 
   200 & 0.014 & 0.001 & 0.001 & 0.001 & 0.001 & 0.074 \\ 
   300 & 0.011 & 0.001 & 0.000 & 0.001 & 0.000 & 0.022 \\ 
   400 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.020 \\ 
   500 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.004 \\ 
   750 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  1000 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
  1500 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Mean penalty/shrinkage parameter by length of time series} 
\label{tab:Chordal:shrink}
\end{table}


==> Tables/Chordal_summary_ll.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:07:09 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rrrrrrrr}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & REAL\_OR\_ML & SHRINKAGE \\ 
  \hline
 25 & -2882.80 & -799.43 & -817.47 & -793.26 & -811.31 & 701.03 & -4200.59 \\ 
   50 & -2232.17 & 241.89 & 238.47 & 229.19 & 229.28 & 768.55 & -3590.65 \\ 
   75 & -1804.68 & 400.90 & 400.83 & 410.29 & 410.23 & 696.69 & -3117.99 \\ 
  100 & -1231.09 & 468.27 & 468.24 & 472.50 & 472.18 & 690.84 & -2643.30 \\ 
  200 & -436.25 & 548.88 & 548.13 & 547.93 & 546.42 & 659.23 & -1277.56 \\ 
  300 & -145.02 & 594.35 & 595.46 & 596.03 & 597.04 & 662.61 & -566.08 \\ 
  400 & -34.19 & 598.96 & 599.91 & 601.84 & 602.07 & 653.18 & -295.88 \\ 
  500 & -3.83 & 580.88 & 580.91 & 582.46 & 582.45 & 620.99 & -69.26 \\ 
  750 & 66.79 & 587.58 & 587.52 & 586.60 & 586.60 & 615.98 & 204.10 \\ 
  1000 & 100.79 & 590.33 & 590.33 & 537.03 & 537.03 & 612.48 & 327.54 \\ 
  1500 & 130.50 & 596.72 & 596.72 & 598.33 & 598.33 & 612.41 & 431.36 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Likelihood of the models. Mean values over 5 distinct training / validation sets and for 10 test set each.} 
\label{tab:Chordal_summary:1}
\end{table}


==> Tables/ClusterGen.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:10:54 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rlrrrrrrr}
  \hline
Series length & Algorithm & Mean Log-likelihood & Stdev Log-likelihood & Mean number of parameters in inverse & Min clique size & Median clique size & Max clique size & Penalty/Shrinkage parameter \\ 
  \hline
 25 & GLASSO\_XVAL & -5191.34 & 39.26 & 484.00 &  &  &  & 0.33 \\ 
   25 & MFCF\_FIX & -4950.18 & 35.17 & 1062.00 & 10.00 & 11.00 & 20.00 & 0.97 \\ 
   25 & MFCF\_FIX\_ID & -4968.61 & 33.86 & 1164.00 & 6.00 & 16.00 & 18.00 & 0.95 \\ 
   25 & MFCF\_VAR & -4995.07 & 12.55 & 234.00 & 4.00 & 13.00 & 20.00 & 0.99 \\ 
   25 & MFCF\_VAR\_ID & -4994.55 & 17.40 & 36.00 & 2.00 & 11.00 & 20.00 & 0.99 \\ 
   25 & REAL\_OR\_ML & -4780.31 & 64.96 & 4950.00 &  &  &  &  \\ 
   25 & SHRINKAGE & -4994.96 & 12.08 & 1414.00 &  &  &  & 0.99 \\ 
   50 & GLASSO\_XVAL & -5064.38 & 62.22 & 459.00 &  &  &  & 0.24 \\ 
   50 & MFCF\_FIX & -4936.61 & 66.74 & 465.00 & 4.00 & 5.00 & 9.00 & 0.97 \\ 
   50 & MFCF\_FIX\_ID & -4953.39 & 55.92 & 679.00 & 3.00 & 8.00 & 15.00 & 0.89 \\ 
   50 & MFCF\_VAR & -4940.76 & 73.55 & 250.00 & 2.00 & 4.00 & 9.00 & 0.97 \\ 
   50 & MFCF\_VAR\_ID & -4976.69 & 25.09 & 276.00 & 2.00 & 13.00 & 20.00 & 0.91 \\ 
   50 & REAL\_OR\_ML & -4788.28 & 96.15 & 4950.00 &  &  &  &  \\ 
   50 & SHRINKAGE & -4990.40 & 25.06 & 1414.00 &  &  &  & 0.99 \\ 
   75 & GLASSO\_XVAL & -5041.48 & 63.48 & 343.00 &  &  &  & 0.22 \\ 
   75 & MFCF\_FIX & -4940.46 & 61.16 & 592.00 & 3.00 & 6.00 & 12.00 & 0.94 \\ 
   75 & MFCF\_FIX\_ID & -4956.52 & 47.66 & 1129.00 & 6.00 & 13.00 & 18.00 & 0.88 \\ 
   75 & MFCF\_VAR & -4947.82 & 57.77 & 255.00 & 3.00 & 5.00 & 6.00 & 0.95 \\ 
   75 & MFCF\_VAR\_ID & -4955.02 & 53.93 & 353.00 & 4.00 & 9.00 & 15.00 & 0.87 \\ 
   75 & REAL\_OR\_ML & -4792.11 & 99.91 & 4950.00 &  &  &  &  \\ 
   75 & SHRINKAGE & -4973.09 & 33.68 & 4950.00 &  &  &  & 0.95 \\ 
  100 & GLASSO\_XVAL & -5000.22 & 58.90 & 472.00 &  &  &  & 0.17 \\ 
  100 & MFCF\_FIX & -4934.51 & 52.58 & 555.00 & 3.00 & 6.00 & 11.00 & 0.88 \\ 
  100 & MFCF\_FIX\_ID & -4945.25 & 50.43 & 757.00 & 3.00 & 10.00 & 14.00 & 0.83 \\ 
  100 & MFCF\_VAR & -4939.14 & 55.83 & 247.00 & 3.00 & 3.00 & 9.00 & 0.90 \\ 
  100 & MFCF\_VAR\_ID & -4969.89 & 31.40 & 308.00 & 5.00 & 12.50 & 20.00 & 0.83 \\ 
  100 & REAL\_OR\_ML & -4804.96 & 83.21 & 4950.00 &  &  &  &  \\ 
  100 & SHRINKAGE & -4966.09 & 33.90 & 4950.00 &  &  &  & 0.93 \\ 
  200 & GLASSO\_XVAL & -4953.33 & 63.31 & 472.00 &  &  &  & 0.12 \\ 
  200 & MFCF\_FIX & -4931.11 & 61.32 & 351.00 & 3.00 & 4.00 & 7.00 & 0.85 \\ 
  200 & MFCF\_FIX\_ID & -4935.99 & 64.07 & 687.00 & 5.00 & 7.00 & 12.00 & 0.75 \\ 
  200 & MFCF\_VAR & -4931.13 & 61.79 & 238.00 & 3.00 & 4.00 & 5.00 & 0.86 \\ 
  200 & MFCF\_VAR\_ID & -4964.09 & 38.35 & 301.00 & 3.00 & 12.00 & 20.00 & 0.77 \\ 
  200 & REAL\_OR\_ML & -4817.97 & 80.17 & 4950.00 &  &  &  &  \\ 
  200 & SHRINKAGE & -4961.06 & 41.28 & 4950.00 &  &  &  & 0.89 \\ 
  300 & GLASSO\_XVAL & -4937.44 & 67.18 & 260.00 &  &  &  & 0.12 \\ 
  300 & MFCF\_FIX & -4915.24 & 67.90 & 352.00 & 4.00 & 5.00 & 5.00 & 0.73 \\ 
  300 & MFCF\_FIX\_ID & -4921.63 & 69.44 & 466.00 & 5.00 & 6.00 & 7.00 & 0.64 \\ 
  300 & MFCF\_VAR & -4916.59 & 71.71 & 272.00 & 3.00 & 4.00 & 6.00 & 0.72 \\ 
  300 & MFCF\_VAR\_ID & -4919.42 & 71.33 & 382.00 & 3.00 & 9.00 & 9.00 & 0.62 \\ 
  300 & REAL\_OR\_ML & -4803.21 & 93.59 & 4950.00 &  &  &  &  \\ 
  300 & SHRINKAGE & -4950.24 & 49.40 & 4950.00 &  &  &  & 0.86 \\ 
  400 & GLASSO\_XVAL & -4939.11 & 62.43 & 155.00 &  &  &  & 0.12 \\ 
  400 & MFCF\_FIX & -4909.28 & 71.68 & 331.00 & 3.00 & 4.00 & 7.00 & 0.63 \\ 
  400 & MFCF\_FIX\_ID & -4912.48 & 71.92 & 369.00 & 3.00 & 4.00 & 8.00 & 0.55 \\ 
  400 & MFCF\_VAR & -4911.22 & 71.17 & 272.00 & 3.00 & 3.00 & 7.00 & 0.63 \\ 
  400 & MFCF\_VAR\_ID & -4911.58 & 71.72 & 343.00 & 3.00 & 4.00 & 8.00 & 0.54 \\ 
  400 & REAL\_OR\_ML & -4807.00 & 88.94 & 4950.00 &  &  &  &  \\ 
  400 & SHRINKAGE & -4945.47 & 54.14 & 4950.00 &  &  &  & 0.84 \\ 
  500 & GLASSO\_XVAL & -4940.11 & 63.55 & 108.00 &  &  &  & 0.12 \\ 
  500 & MFCF\_FIX & -4905.04 & 75.13 & 294.00 & 3.00 & 4.00 & 5.00 & 0.56 \\ 
  500 & MFCF\_FIX\_ID & -4906.25 & 74.64 & 351.00 & 3.00 & 5.00 & 6.00 & 0.48 \\ 
  500 & MFCF\_VAR & -4905.42 & 74.47 & 297.00 & 3.00 & 4.00 & 7.00 & 0.54 \\ 
  500 & MFCF\_VAR\_ID & -4905.42 & 75.20 & 364.00 & 3.00 & 5.00 & 10.00 & 0.46 \\ 
  500 & REAL\_OR\_ML & -4811.13 & 88.05 & 4950.00 &  &  &  &  \\ 
  500 & SHRINKAGE & -4942.50 & 54.50 & 4950.00 &  &  &  & 0.80 \\ 
  750 & GLASSO\_XVAL & -4926.24 & 78.47 & 165.00 &  &  &  & 0.10 \\ 
  750 & MFCF\_FIX & -4898.56 & 72.71 & 370.00 & 3.00 & 5.00 & 7.00 & 0.40 \\ 
  750 & MFCF\_FIX\_ID & -4898.35 & 74.58 & 408.00 & 3.00 & 5.00 & 7.00 & 0.36 \\ 
  750 & MFCF\_VAR & -4897.93 & 74.96 & 330.00 & 3.00 & 4.00 & 7.00 & 0.39 \\ 
  750 & MFCF\_VAR\_ID & -4897.05 & 76.17 & 428.00 & 4.00 & 7.00 & 16.00 & 0.38 \\ 
  750 & REAL\_OR\_ML & -4814.85 & 84.14 & 4950.00 &  &  &  &  \\ 
  750 & SHRINKAGE & -4935.09 & 56.08 & 4950.00 &  &  &  & 0.76 \\ 
  1000 & GLASSO\_XVAL & -4915.43 & 61.60 & 171.00 &  &  &  & 0.08 \\ 
  1000 & MFCF\_FIX & -4896.66 & 71.25 & 313.00 & 3.00 & 4.00 & 6.00 & 0.34 \\ 
  1000 & MFCF\_FIX\_ID & -4896.88 & 72.76 & 427.00 & 3.00 & 6.00 & 7.00 & 0.31 \\ 
  1000 & MFCF\_VAR & -4895.81 & 71.02 & 292.00 & 3.00 & 4.00 & 6.00 & 0.32 \\ 
  1000 & MFCF\_VAR\_ID & -4895.43 & 72.20 & 336.00 & 3.00 & 5.00 & 7.00 & 0.28 \\ 
  1000 & REAL\_OR\_ML & -4821.58 & 80.27 & 4950.00 &  &  &  &  \\ 
  1000 & SHRINKAGE & -4930.52 & 56.76 & 4950.00 &  &  &  & 0.71 \\ 
  1500 & GLASSO\_XVAL & -4897.12 & 81.69 & 922.00 &  &  &  & 0.05 \\ 
  1500 & MFCF\_FIX & -4884.08 & 78.83 & 313.00 & 3.00 & 4.00 & 6.00 & 0.20 \\ 
  1500 & MFCF\_FIX\_ID & -4884.36 & 78.90 & 313.00 & 3.00 & 4.00 & 6.00 & 0.18 \\ 
  1500 & MFCF\_VAR & -4883.96 & 78.75 & 282.00 & 3.00 & 4.00 & 6.00 & 0.20 \\ 
  1500 & MFCF\_VAR\_ID & -4883.73 & 78.56 & 349.00 & 3.00 & 4.00 & 8.00 & 0.18 \\ 
  1500 & REAL\_OR\_ML & -4819.57 & 83.45 & 4950.00 &  &  &  &  \\ 
  1500 & SHRINKAGE & -4920.63 & 61.58 & 4950.00 &  &  &  & 0.62 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Likelihood of the models. Mean values over 5 distinct training / validation sets and for 10 test set each.} 
\label{tab:ClusterGen:1}
\end{table}


==> Tables/ClusterGen_acc.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:10:54 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rlrrrrrrr}
  \hline
Series length & Algorithm & Mean Log-likelihood & Stdev Log-likelihood & Mean number of parameters in inverse & Min clique size & Median clique size & Max clique size & Penalty/Shrinkage parameter \\ 
  \hline
 25 & GLASSO\_XVAL & -5191.34 & 39.26 & 484.00 &  &  &  & 0.33 \\ 
   25 & MFCF\_FIX & -4950.18 & 35.17 & 1062.00 & 10.00 & 11.00 & 20.00 & 0.97 \\ 
   25 & MFCF\_FIX\_ID & -4968.61 & 33.86 & 1164.00 & 6.00 & 16.00 & 18.00 & 0.95 \\ 
   25 & MFCF\_VAR & -4995.07 & 12.55 & 234.00 & 4.00 & 13.00 & 20.00 & 0.99 \\ 
   25 & MFCF\_VAR\_ID & -4994.55 & 17.40 & 36.00 & 2.00 & 11.00 & 20.00 & 0.99 \\ 
   25 & REAL\_OR\_ML & -4780.31 & 64.96 & 4950.00 &  &  &  &  \\ 
   25 & SHRINKAGE & -4994.96 & 12.08 & 1414.00 &  &  &  & 0.99 \\ 
   50 & GLASSO\_XVAL & -5064.38 & 62.22 & 459.00 &  &  &  & 0.24 \\ 
   50 & MFCF\_FIX & -4936.61 & 66.74 & 465.00 & 4.00 & 5.00 & 9.00 & 0.97 \\ 
   50 & MFCF\_FIX\_ID & -4953.39 & 55.92 & 679.00 & 3.00 & 8.00 & 15.00 & 0.89 \\ 
   50 & MFCF\_VAR & -4940.76 & 73.55 & 250.00 & 2.00 & 4.00 & 9.00 & 0.97 \\ 
   50 & MFCF\_VAR\_ID & -4976.69 & 25.09 & 276.00 & 2.00 & 13.00 & 20.00 & 0.91 \\ 
   50 & REAL\_OR\_ML & -4788.28 & 96.15 & 4950.00 &  &  &  &  \\ 
   50 & SHRINKAGE & -4990.40 & 25.06 & 1414.00 &  &  &  & 0.99 \\ 
   75 & GLASSO\_XVAL & -5041.48 & 63.48 & 343.00 &  &  &  & 0.22 \\ 
   75 & MFCF\_FIX & -4940.46 & 61.16 & 592.00 & 3.00 & 6.00 & 12.00 & 0.94 \\ 
   75 & MFCF\_FIX\_ID & -4956.52 & 47.66 & 1129.00 & 6.00 & 13.00 & 18.00 & 0.88 \\ 
   75 & MFCF\_VAR & -4947.82 & 57.77 & 255.00 & 3.00 & 5.00 & 6.00 & 0.95 \\ 
   75 & MFCF\_VAR\_ID & -4955.02 & 53.93 & 353.00 & 4.00 & 9.00 & 15.00 & 0.87 \\ 
   75 & REAL\_OR\_ML & -4792.11 & 99.91 & 4950.00 &  &  &  &  \\ 
   75 & SHRINKAGE & -4973.09 & 33.68 & 4950.00 &  &  &  & 0.95 \\ 
  100 & GLASSO\_XVAL & -5000.22 & 58.90 & 472.00 &  &  &  & 0.17 \\ 
  100 & MFCF\_FIX & -4934.51 & 52.58 & 555.00 & 3.00 & 6.00 & 11.00 & 0.88 \\ 
  100 & MFCF\_FIX\_ID & -4945.25 & 50.43 & 757.00 & 3.00 & 10.00 & 14.00 & 0.83 \\ 
  100 & MFCF\_VAR & -4939.14 & 55.83 & 247.00 & 3.00 & 3.00 & 9.00 & 0.90 \\ 
  100 & MFCF\_VAR\_ID & -4969.89 & 31.40 & 308.00 & 5.00 & 12.50 & 20.00 & 0.83 \\ 
  100 & REAL\_OR\_ML & -4804.96 & 83.21 & 4950.00 &  &  &  &  \\ 
  100 & SHRINKAGE & -4966.09 & 33.90 & 4950.00 &  &  &  & 0.93 \\ 
  200 & GLASSO\_XVAL & -4953.33 & 63.31 & 472.00 &  &  &  & 0.12 \\ 
  200 & MFCF\_FIX & -4931.11 & 61.32 & 351.00 & 3.00 & 4.00 & 7.00 & 0.85 \\ 
  200 & MFCF\_FIX\_ID & -4935.99 & 64.07 & 687.00 & 5.00 & 7.00 & 12.00 & 0.75 \\ 
  200 & MFCF\_VAR & -4931.13 & 61.79 & 238.00 & 3.00 & 4.00 & 5.00 & 0.86 \\ 
  200 & MFCF\_VAR\_ID & -4964.09 & 38.35 & 301.00 & 3.00 & 12.00 & 20.00 & 0.77 \\ 
  200 & REAL\_OR\_ML & -4817.97 & 80.17 & 4950.00 &  &  &  &  \\ 
  200 & SHRINKAGE & -4961.06 & 41.28 & 4950.00 &  &  &  & 0.89 \\ 
  300 & GLASSO\_XVAL & -4937.44 & 67.18 & 260.00 &  &  &  & 0.12 \\ 
  300 & MFCF\_FIX & -4915.24 & 67.90 & 352.00 & 4.00 & 5.00 & 5.00 & 0.73 \\ 
  300 & MFCF\_FIX\_ID & -4921.63 & 69.44 & 466.00 & 5.00 & 6.00 & 7.00 & 0.64 \\ 
  300 & MFCF\_VAR & -4916.59 & 71.71 & 272.00 & 3.00 & 4.00 & 6.00 & 0.72 \\ 
  300 & MFCF\_VAR\_ID & -4919.42 & 71.33 & 382.00 & 3.00 & 9.00 & 9.00 & 0.62 \\ 
  300 & REAL\_OR\_ML & -4803.21 & 93.59 & 4950.00 &  &  &  &  \\ 
  300 & SHRINKAGE & -4950.24 & 49.40 & 4950.00 &  &  &  & 0.86 \\ 
  400 & GLASSO\_XVAL & -4939.11 & 62.43 & 155.00 &  &  &  & 0.12 \\ 
  400 & MFCF\_FIX & -4909.28 & 71.68 & 331.00 & 3.00 & 4.00 & 7.00 & 0.63 \\ 
  400 & MFCF\_FIX\_ID & -4912.48 & 71.92 & 369.00 & 3.00 & 4.00 & 8.00 & 0.55 \\ 
  400 & MFCF\_VAR & -4911.22 & 71.17 & 272.00 & 3.00 & 3.00 & 7.00 & 0.63 \\ 
  400 & MFCF\_VAR\_ID & -4911.58 & 71.72 & 343.00 & 3.00 & 4.00 & 8.00 & 0.54 \\ 
  400 & REAL\_OR\_ML & -4807.00 & 88.94 & 4950.00 &  &  &  &  \\ 
  400 & SHRINKAGE & -4945.47 & 54.14 & 4950.00 &  &  &  & 0.84 \\ 
  500 & GLASSO\_XVAL & -4940.11 & 63.55 & 108.00 &  &  &  & 0.12 \\ 
  500 & MFCF\_FIX & -4905.04 & 75.13 & 294.00 & 3.00 & 4.00 & 5.00 & 0.56 \\ 
  500 & MFCF\_FIX\_ID & -4906.25 & 74.64 & 351.00 & 3.00 & 5.00 & 6.00 & 0.48 \\ 
  500 & MFCF\_VAR & -4905.42 & 74.47 & 297.00 & 3.00 & 4.00 & 7.00 & 0.54 \\ 
  500 & MFCF\_VAR\_ID & -4905.42 & 75.20 & 364.00 & 3.00 & 5.00 & 10.00 & 0.46 \\ 
  500 & REAL\_OR\_ML & -4811.13 & 88.05 & 4950.00 &  &  &  &  \\ 
  500 & SHRINKAGE & -4942.50 & 54.50 & 4950.00 &  &  &  & 0.80 \\ 
  750 & GLASSO\_XVAL & -4926.24 & 78.47 & 165.00 &  &  &  & 0.10 \\ 
  750 & MFCF\_FIX & -4898.56 & 72.71 & 370.00 & 3.00 & 5.00 & 7.00 & 0.40 \\ 
  750 & MFCF\_FIX\_ID & -4898.35 & 74.58 & 408.00 & 3.00 & 5.00 & 7.00 & 0.36 \\ 
  750 & MFCF\_VAR & -4897.93 & 74.96 & 330.00 & 3.00 & 4.00 & 7.00 & 0.39 \\ 
  750 & MFCF\_VAR\_ID & -4897.05 & 76.17 & 428.00 & 4.00 & 7.00 & 16.00 & 0.38 \\ 
  750 & REAL\_OR\_ML & -4814.85 & 84.14 & 4950.00 &  &  &  &  \\ 
  750 & SHRINKAGE & -4935.09 & 56.08 & 4950.00 &  &  &  & 0.76 \\ 
  1000 & GLASSO\_XVAL & -4915.43 & 61.60 & 171.00 &  &  &  & 0.08 \\ 
  1000 & MFCF\_FIX & -4896.66 & 71.25 & 313.00 & 3.00 & 4.00 & 6.00 & 0.34 \\ 
  1000 & MFCF\_FIX\_ID & -4896.88 & 72.76 & 427.00 & 3.00 & 6.00 & 7.00 & 0.31 \\ 
  1000 & MFCF\_VAR & -4895.81 & 71.02 & 292.00 & 3.00 & 4.00 & 6.00 & 0.32 \\ 
  1000 & MFCF\_VAR\_ID & -4895.43 & 72.20 & 336.00 & 3.00 & 5.00 & 7.00 & 0.28 \\ 
  1000 & REAL\_OR\_ML & -4821.58 & 80.27 & 4950.00 &  &  &  &  \\ 
  1000 & SHRINKAGE & -4930.52 & 56.76 & 4950.00 &  &  &  & 0.71 \\ 
  1500 & GLASSO\_XVAL & -4897.12 & 81.69 & 922.00 &  &  &  & 0.05 \\ 
  1500 & MFCF\_FIX & -4884.08 & 78.83 & 313.00 & 3.00 & 4.00 & 6.00 & 0.20 \\ 
  1500 & MFCF\_FIX\_ID & -4884.36 & 78.90 & 313.00 & 3.00 & 4.00 & 6.00 & 0.18 \\ 
  1500 & MFCF\_VAR & -4883.96 & 78.75 & 282.00 & 3.00 & 4.00 & 6.00 & 0.20 \\ 
  1500 & MFCF\_VAR\_ID & -4883.73 & 78.56 & 349.00 & 3.00 & 4.00 & 8.00 & 0.18 \\ 
  1500 & REAL\_OR\_ML & -4819.57 & 83.45 & 4950.00 &  &  &  &  \\ 
  1500 & SHRINKAGE & -4920.63 & 61.58 & 4950.00 &  &  &  & 0.62 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Performance of the models on a random clique forest. Mean values over 10 sample runs.} 
\label{tab:ClusterGen:2}
\end{table}


==> Tables/ClusterGen_paramno.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:11:00 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{|r|R{2cm}|R{2cm}|R{2cm}|R{2cm}|R{2cm}|R{2cm}|}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & SHRINKAGE \\ 
  \hline
25 & 484 & 1062 & 1164 & 234 & 36 & 1414 \\ 
  50 & 459 & 465 & 679 & 250 & 276 & 1414 \\ 
  75 & 343 & 592 & 1129 & 255 & 353 & 4950 \\ 
  100 & 472 & 555 & 757 & 247 & 308 & 4950 \\ 
  200 & 472 & 351 & 687 & 238 & 301 & 4950 \\ 
  300 & 260 & 352 & 466 & 272 & 382 & 4950 \\ 
  400 & 155 & 331 & 369 & 272 & 343 & 4950 \\ 
  500 & 108 & 294 & 351 & 297 & 364 & 4950 \\ 
  750 & 165 & 370 & 408 & 330 & 428 & 4950 \\ 
  1000 & 171 & 313 & 427 & 292 & 336 & 4950 \\ 
  1500 & 922 & 313 & 313 & 282 & 349 & 4950 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Mean number of non-zero coefficient in the precision matrix by length of time series} 
\label{tab:ClusterGen:param_no}
\end{table}


==> Tables/ClusterGen_shrink.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:11:00 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{|r|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & SHRINKAGE \\ 
  \hline
  25 & 0.333 & 0.966 & 0.950 & 0.992 & 0.987 & 0.993 \\ 
    50 & 0.241 & 0.966 & 0.893 & 0.967 & 0.912 & 0.986 \\ 
    75 & 0.218 & 0.940 & 0.883 & 0.949 & 0.866 & 0.949 \\ 
   100 & 0.171 & 0.883 & 0.826 & 0.901 & 0.829 & 0.929 \\ 
   200 & 0.123 & 0.855 & 0.754 & 0.860 & 0.766 & 0.892 \\ 
   300 & 0.120 & 0.734 & 0.644 & 0.721 & 0.625 & 0.864 \\ 
   400 & 0.120 & 0.629 & 0.546 & 0.629 & 0.539 & 0.837 \\ 
   500 & 0.120 & 0.556 & 0.485 & 0.543 & 0.465 & 0.805 \\ 
   750 & 0.103 & 0.399 & 0.364 & 0.389 & 0.376 & 0.755 \\ 
  1000 & 0.081 & 0.339 & 0.312 & 0.321 & 0.280 & 0.713 \\ 
  1500 & 0.053 & 0.203 & 0.184 & 0.197 & 0.180 & 0.622 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Mean penalty/shrinkage parameter by length of time series} 
\label{tab:ClusterGen:shrink}
\end{table}


==> Tables/Factor.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:09:52 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rlrrrrrrr}
  \hline
Series length & Algorithm & Mean Log-likelihood & Stdev Log-likelihood & Mean number of parameters in inverse & Min clique size & Median clique size & Max clique size & Penalty/Shrinkage parameter \\ 
  \hline
 25 & GLASSO\_XVAL & 61.12 & 160.23 & 1168.00 &  &  &  & 0.12 \\ 
   25 & MFCF\_FIX & -313.06 & 228.45 & 1694.00 & 19.00 &  20 & 20.00 & 0.27 \\ 
   25 & MFCF\_FIX\_ID & -279.57 & 216.88 & 1661.00 & 18.00 &  20 & 20.00 & 0.26 \\ 
   25 & MFCF\_VAR & -341.81 & 261.74 & 1582.00 & 17.00 &  19 & 19.00 & 0.25 \\ 
   25 & MFCF\_VAR\_ID & -334.90 & 263.74 & 1597.00 & 17.00 &  19 & 20.00 & 0.25 \\ 
   25 & REAL\_OR\_ML & 1739.32 & 145.98 & 4950.00 &  &  &  &  \\ 
   25 & SHRINKAGE & 252.30 & 210.92 & 4950.00 &  &  &  & 0.30 \\ 
   50 & GLASSO\_XVAL & 112.32 & 84.78 & 1206.00 &  &  &  & 0.12 \\ 
   50 & MFCF\_FIX & 53.73 & 136.25 & 1677.00 & 18.00 &  20 & 20.00 & 0.19 \\ 
   50 & MFCF\_FIX\_ID & 81.22 & 134.66 & 1661.00 & 18.00 &  20 & 20.00 & 0.18 \\ 
   50 & MFCF\_VAR & 114.91 & 143.67 & 1694.00 & 19.00 &  20 & 20.00 & 0.18 \\ 
   50 & MFCF\_VAR\_ID & 119.88 & 149.89 & 1694.00 & 19.00 &  20 & 20.00 & 0.18 \\ 
   50 & REAL\_OR\_ML & 1614.94 & 79.39 & 4950.00 &  &  &  &  \\ 
   50 & SHRINKAGE & 552.55 & 136.14 & 4950.00 &  &  &  & 0.23 \\ 
   75 & GLASSO\_XVAL & 450.13 & 132.34 & 1308.00 &  &  &  & 0.09 \\ 
   75 & MFCF\_FIX & 233.31 & 116.31 & 1661.00 & 19.00 &  19 & 20.00 & 0.15 \\ 
   75 & MFCF\_FIX\_ID & 265.18 & 115.11 & 1661.00 & 19.00 &  19 & 20.00 & 0.14 \\ 
   75 & MFCF\_VAR & 265.91 & 99.18 & 1678.00 & 19.00 &  20 & 20.00 & 0.15 \\ 
   75 & MFCF\_VAR\_ID & 268.30 & 96.85 & 1678.00 & 19.00 &  20 & 20.00 & 0.15 \\ 
   75 & REAL\_OR\_ML & 1558.30 & 57.91 & 4950.00 &  &  &  &  \\ 
   75 & SHRINKAGE & 713.32 & 107.60 & 4950.00 &  &  &  & 0.20 \\ 
  100 & GLASSO\_XVAL & 812.10 & 281.35 & 1648.00 &  &  &  & 0.06 \\ 
  100 & MFCF\_FIX & 398.28 & 84.86 & 1710.00 & 20.00 &  20 & 20.00 & 0.13 \\ 
  100 & MFCF\_FIX\_ID & 405.97 & 86.05 & 1710.00 & 20.00 &  20 & 20.00 & 0.13 \\ 
  100 & MFCF\_VAR & 417.36 & 83.15 & 1645.00 & 19.00 &  19 & 20.00 & 0.12 \\ 
  100 & MFCF\_VAR\_ID & 419.41 & 78.47 & 1645.00 & 19.00 &  19 & 20.00 & 0.12 \\ 
  100 & REAL\_OR\_ML & 1523.66 & 102.41 & 4950.00 &  &  &  &  \\ 
  100 & SHRINKAGE & 789.05 & 124.56 & 4950.00 &  &  &  & 0.18 \\ 
  200 & GLASSO\_XVAL & 1200.52 & 45.70 & 2143.00 &  &  &  & 0.02 \\ 
  200 & MFCF\_FIX & 595.80 & 15.16 & 1710.00 & 20.00 &  20 & 20.00 & 0.08 \\ 
  200 & MFCF\_FIX\_ID & 602.64 & 15.34 & 1710.00 & 20.00 &  20 & 20.00 & 0.08 \\ 
  200 & MFCF\_VAR & 627.05 & 78.43 & 1678.00 & 19.00 &  20 & 20.00 & 0.08 \\ 
  200 & MFCF\_VAR\_ID & 627.55 & 78.79 & 1694.00 & 19.00 &  20 & 20.00 & 0.08 \\ 
  200 & REAL\_OR\_ML & 1497.52 & 51.15 & 4950.00 &  &  &  &  \\ 
  200 & SHRINKAGE & 1028.57 & 48.55 & 4950.00 &  &  &  & 0.14 \\ 
  300 & GLASSO\_XVAL & 1334.60 & 64.85 & 2426.00 &  &  &  & 0.01 \\ 
  300 & MFCF\_FIX & 759.23 & 51.23 & 1710.00 & 20.00 &  20 & 20.00 & 0.06 \\ 
  300 & MFCF\_FIX\_ID & 764.49 & 51.08 & 1694.00 & 19.00 &  20 & 20.00 & 0.06 \\ 
  300 & MFCF\_VAR & 696.99 & 81.64 & 1694.00 & 19.00 &  20 & 20.00 & 0.06 \\ 
  300 & MFCF\_VAR\_ID & 697.17 & 81.71 & 1694.00 & 19.00 &  20 & 20.00 & 0.06 \\ 
  300 & REAL\_OR\_ML & 1511.88 & 42.96 & 4950.00 &  &  &  &  \\ 
  300 & SHRINKAGE & 1190.94 & 72.99 & 4950.00 &  &  &  & 0.11 \\ 
  400 & GLASSO\_XVAL & 1357.39 & 46.37 & 2568.00 &  &  &  & 0.01 \\ 
  400 & MFCF\_FIX & 780.88 & 62.62 & 1710.00 & 20.00 &  20 & 20.00 & 0.05 \\ 
  400 & MFCF\_FIX\_ID & 784.18 & 64.00 & 1710.00 & 20.00 &  20 & 20.00 & 0.05 \\ 
  400 & MFCF\_VAR & 728.48 & 61.37 & 1710.00 & 20.00 &  20 & 20.00 & 0.05 \\ 
  400 & MFCF\_VAR\_ID & 728.49 & 61.67 & 1710.00 & 20.00 &  20 & 20.00 & 0.05 \\ 
  400 & REAL\_OR\_ML & 1489.11 & 40.60 & 4950.00 &  &  &  &  \\ 
  400 & SHRINKAGE & 1241.16 & 45.80 & 4950.00 &  &  &  & 0.09 \\ 
  500 & GLASSO\_XVAL & 1350.93 & 45.37 & 2814.00 &  &  &  & 0.01 \\ 
  500 & MFCF\_FIX & 757.01 & 76.79 & 1694.00 & 19.00 &  20 & 20.00 & 0.04 \\ 
  500 & MFCF\_FIX\_ID & 758.04 & 76.52 & 1694.00 & 19.00 &  20 & 20.00 & 0.04 \\ 
  500 & MFCF\_VAR & 755.60 & 48.11 & 1694.00 & 19.00 &  20 & 20.00 & 0.04 \\ 
  500 & MFCF\_VAR\_ID & 755.42 & 47.85 & 1694.00 & 19.00 &  20 & 20.00 & 0.04 \\ 
  500 & REAL\_OR\_ML & 1448.57 & 36.20 & 4950.00 &  &  &  &  \\ 
  500 & SHRINKAGE & 1265.29 & 44.32 & 4950.00 &  &  &  & 0.08 \\ 
  750 & GLASSO\_XVAL & 1390.70 & 54.58 & 2760.00 &  &  &  & 0.01 \\ 
  750 & MFCF\_FIX & 788.34 & 55.71 & 1694.00 & 19.00 &  20 & 20.00 & 0.03 \\ 
  750 & MFCF\_FIX\_ID & 788.87 & 55.55 & 1694.00 & 19.00 &  20 & 20.00 & 0.03 \\ 
  750 & MFCF\_VAR & 770.07 & 48.19 & 1694.00 & 19.00 &  20 & 20.00 & 0.03 \\ 
  750 & MFCF\_VAR\_ID & 770.16 & 48.10 & 1694.00 & 19.00 &  20 & 20.00 & 0.03 \\ 
  750 & REAL\_OR\_ML & 1434.73 & 42.36 & 4950.00 &  &  &  &  \\ 
  750 & SHRINKAGE & 1356.34 & 51.04 & 4950.00 &  &  &  & 0.06 \\ 
  1000 & GLASSO\_XVAL & 1444.52 & 44.06 & 2755.00 &  &  &  & 0.01 \\ 
  1000 & MFCF\_FIX & 852.73 & 40.88 & 1710.00 & 20.00 &  20 & 20.00 & 0.02 \\ 
  1000 & MFCF\_FIX\_ID & 853.14 & 41.14 & 1710.00 & 20.00 &  20 & 20.00 & 0.02 \\ 
  1000 & MFCF\_VAR & 816.86 & 68.74 & 1678.00 & 19.00 &  20 & 20.00 & 0.02 \\ 
  1000 & MFCF\_VAR\_ID & 816.84 & 68.66 & 1678.00 & 19.00 &  20 & 20.00 & 0.02 \\ 
  1000 & REAL\_OR\_ML & 1465.82 & 42.79 & 4950.00 &  &  &  &  \\ 
  1000 & SHRINKAGE & 1438.18 & 47.20 & 4950.00 &  &  &  & 0.04 \\ 
  1500 & GLASSO\_XVAL & 1427.13 & 12.36 & 2761.00 &  &  &  & 0.01 \\ 
  1500 & MFCF\_FIX & 867.20 & 35.90 & 1694.00 & 19.00 &  20 & 20.00 & 0.01 \\ 
  1500 & MFCF\_FIX\_ID & 867.38 & 35.82 & 1694.00 & 19.00 &  20 & 20.00 & 0.01 \\ 
  1500 & MFCF\_VAR & 815.21 & 42.09 & 1710.00 & 20.00 &  20 & 20.00 & 0.01 \\ 
  1500 & MFCF\_VAR\_ID & 815.28 & 42.04 & 1710.00 & 20.00 &  20 & 20.00 & 0.01 \\ 
  1500 & REAL\_OR\_ML & 1429.06 & 12.51 & 4950.00 &  &  &  &  \\ 
  1500 & SHRINKAGE & 1455.53 & 16.91 & 4950.00 &  &  &  & 0.04 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Likelihood of the models. Mean values over 5 distinct training / validation sets and for 10 test set each.} 
\label{tab:Factor:1}
\end{table}


==> Tables/Factor_acc.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:09:52 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rlrrrrrrr}
  \hline
Series length & Algorithm & Mean Log-likelihood & Stdev Log-likelihood & Mean number of parameters in inverse & Min clique size & Median clique size & Max clique size & Penalty/Shrinkage parameter \\ 
  \hline
 25 & GLASSO\_XVAL & 61.12 & 160.23 & 1168.00 &  &  &  & 0.12 \\ 
   25 & MFCF\_FIX & -313.06 & 228.45 & 1694.00 & 19.00 &  20 & 20.00 & 0.27 \\ 
   25 & MFCF\_FIX\_ID & -279.57 & 216.88 & 1661.00 & 18.00 &  20 & 20.00 & 0.26 \\ 
   25 & MFCF\_VAR & -341.81 & 261.74 & 1582.00 & 17.00 &  19 & 19.00 & 0.25 \\ 
   25 & MFCF\_VAR\_ID & -334.90 & 263.74 & 1597.00 & 17.00 &  19 & 20.00 & 0.25 \\ 
   25 & REAL\_OR\_ML & 1739.32 & 145.98 & 4950.00 &  &  &  &  \\ 
   25 & SHRINKAGE & 252.30 & 210.92 & 4950.00 &  &  &  & 0.30 \\ 
   50 & GLASSO\_XVAL & 112.32 & 84.78 & 1206.00 &  &  &  & 0.12 \\ 
   50 & MFCF\_FIX & 53.73 & 136.25 & 1677.00 & 18.00 &  20 & 20.00 & 0.19 \\ 
   50 & MFCF\_FIX\_ID & 81.22 & 134.66 & 1661.00 & 18.00 &  20 & 20.00 & 0.18 \\ 
   50 & MFCF\_VAR & 114.91 & 143.67 & 1694.00 & 19.00 &  20 & 20.00 & 0.18 \\ 
   50 & MFCF\_VAR\_ID & 119.88 & 149.89 & 1694.00 & 19.00 &  20 & 20.00 & 0.18 \\ 
   50 & REAL\_OR\_ML & 1614.94 & 79.39 & 4950.00 &  &  &  &  \\ 
   50 & SHRINKAGE & 552.55 & 136.14 & 4950.00 &  &  &  & 0.23 \\ 
   75 & GLASSO\_XVAL & 450.13 & 132.34 & 1308.00 &  &  &  & 0.09 \\ 
   75 & MFCF\_FIX & 233.31 & 116.31 & 1661.00 & 19.00 &  19 & 20.00 & 0.15 \\ 
   75 & MFCF\_FIX\_ID & 265.18 & 115.11 & 1661.00 & 19.00 &  19 & 20.00 & 0.14 \\ 
   75 & MFCF\_VAR & 265.91 & 99.18 & 1678.00 & 19.00 &  20 & 20.00 & 0.15 \\ 
   75 & MFCF\_VAR\_ID & 268.30 & 96.85 & 1678.00 & 19.00 &  20 & 20.00 & 0.15 \\ 
   75 & REAL\_OR\_ML & 1558.30 & 57.91 & 4950.00 &  &  &  &  \\ 
   75 & SHRINKAGE & 713.32 & 107.60 & 4950.00 &  &  &  & 0.20 \\ 
  100 & GLASSO\_XVAL & 812.10 & 281.35 & 1648.00 &  &  &  & 0.06 \\ 
  100 & MFCF\_FIX & 398.28 & 84.86 & 1710.00 & 20.00 &  20 & 20.00 & 0.13 \\ 
  100 & MFCF\_FIX\_ID & 405.97 & 86.05 & 1710.00 & 20.00 &  20 & 20.00 & 0.13 \\ 
  100 & MFCF\_VAR & 417.36 & 83.15 & 1645.00 & 19.00 &  19 & 20.00 & 0.12 \\ 
  100 & MFCF\_VAR\_ID & 419.41 & 78.47 & 1645.00 & 19.00 &  19 & 20.00 & 0.12 \\ 
  100 & REAL\_OR\_ML & 1523.66 & 102.41 & 4950.00 &  &  &  &  \\ 
  100 & SHRINKAGE & 789.05 & 124.56 & 4950.00 &  &  &  & 0.18 \\ 
  200 & GLASSO\_XVAL & 1200.52 & 45.70 & 2143.00 &  &  &  & 0.02 \\ 
  200 & MFCF\_FIX & 595.80 & 15.16 & 1710.00 & 20.00 &  20 & 20.00 & 0.08 \\ 
  200 & MFCF\_FIX\_ID & 602.64 & 15.34 & 1710.00 & 20.00 &  20 & 20.00 & 0.08 \\ 
  200 & MFCF\_VAR & 627.05 & 78.43 & 1678.00 & 19.00 &  20 & 20.00 & 0.08 \\ 
  200 & MFCF\_VAR\_ID & 627.55 & 78.79 & 1694.00 & 19.00 &  20 & 20.00 & 0.08 \\ 
  200 & REAL\_OR\_ML & 1497.52 & 51.15 & 4950.00 &  &  &  &  \\ 
  200 & SHRINKAGE & 1028.57 & 48.55 & 4950.00 &  &  &  & 0.14 \\ 
  300 & GLASSO\_XVAL & 1334.60 & 64.85 & 2426.00 &  &  &  & 0.01 \\ 
  300 & MFCF\_FIX & 759.23 & 51.23 & 1710.00 & 20.00 &  20 & 20.00 & 0.06 \\ 
  300 & MFCF\_FIX\_ID & 764.49 & 51.08 & 1694.00 & 19.00 &  20 & 20.00 & 0.06 \\ 
  300 & MFCF\_VAR & 696.99 & 81.64 & 1694.00 & 19.00 &  20 & 20.00 & 0.06 \\ 
  300 & MFCF\_VAR\_ID & 697.17 & 81.71 & 1694.00 & 19.00 &  20 & 20.00 & 0.06 \\ 
  300 & REAL\_OR\_ML & 1511.88 & 42.96 & 4950.00 &  &  &  &  \\ 
  300 & SHRINKAGE & 1190.94 & 72.99 & 4950.00 &  &  &  & 0.11 \\ 
  400 & GLASSO\_XVAL & 1357.39 & 46.37 & 2568.00 &  &  &  & 0.01 \\ 
  400 & MFCF\_FIX & 780.88 & 62.62 & 1710.00 & 20.00 &  20 & 20.00 & 0.05 \\ 
  400 & MFCF\_FIX\_ID & 784.18 & 64.00 & 1710.00 & 20.00 &  20 & 20.00 & 0.05 \\ 
  400 & MFCF\_VAR & 728.48 & 61.37 & 1710.00 & 20.00 &  20 & 20.00 & 0.05 \\ 
  400 & MFCF\_VAR\_ID & 728.49 & 61.67 & 1710.00 & 20.00 &  20 & 20.00 & 0.05 \\ 
  400 & REAL\_OR\_ML & 1489.11 & 40.60 & 4950.00 &  &  &  &  \\ 
  400 & SHRINKAGE & 1241.16 & 45.80 & 4950.00 &  &  &  & 0.09 \\ 
  500 & GLASSO\_XVAL & 1350.93 & 45.37 & 2814.00 &  &  &  & 0.01 \\ 
  500 & MFCF\_FIX & 757.01 & 76.79 & 1694.00 & 19.00 &  20 & 20.00 & 0.04 \\ 
  500 & MFCF\_FIX\_ID & 758.04 & 76.52 & 1694.00 & 19.00 &  20 & 20.00 & 0.04 \\ 
  500 & MFCF\_VAR & 755.60 & 48.11 & 1694.00 & 19.00 &  20 & 20.00 & 0.04 \\ 
  500 & MFCF\_VAR\_ID & 755.42 & 47.85 & 1694.00 & 19.00 &  20 & 20.00 & 0.04 \\ 
  500 & REAL\_OR\_ML & 1448.57 & 36.20 & 4950.00 &  &  &  &  \\ 
  500 & SHRINKAGE & 1265.29 & 44.32 & 4950.00 &  &  &  & 0.08 \\ 
  750 & GLASSO\_XVAL & 1390.70 & 54.58 & 2760.00 &  &  &  & 0.01 \\ 
  750 & MFCF\_FIX & 788.34 & 55.71 & 1694.00 & 19.00 &  20 & 20.00 & 0.03 \\ 
  750 & MFCF\_FIX\_ID & 788.87 & 55.55 & 1694.00 & 19.00 &  20 & 20.00 & 0.03 \\ 
  750 & MFCF\_VAR & 770.07 & 48.19 & 1694.00 & 19.00 &  20 & 20.00 & 0.03 \\ 
  750 & MFCF\_VAR\_ID & 770.16 & 48.10 & 1694.00 & 19.00 &  20 & 20.00 & 0.03 \\ 
  750 & REAL\_OR\_ML & 1434.73 & 42.36 & 4950.00 &  &  &  &  \\ 
  750 & SHRINKAGE & 1356.34 & 51.04 & 4950.00 &  &  &  & 0.06 \\ 
  1000 & GLASSO\_XVAL & 1444.52 & 44.06 & 2755.00 &  &  &  & 0.01 \\ 
  1000 & MFCF\_FIX & 852.73 & 40.88 & 1710.00 & 20.00 &  20 & 20.00 & 0.02 \\ 
  1000 & MFCF\_FIX\_ID & 853.14 & 41.14 & 1710.00 & 20.00 &  20 & 20.00 & 0.02 \\ 
  1000 & MFCF\_VAR & 816.86 & 68.74 & 1678.00 & 19.00 &  20 & 20.00 & 0.02 \\ 
  1000 & MFCF\_VAR\_ID & 816.84 & 68.66 & 1678.00 & 19.00 &  20 & 20.00 & 0.02 \\ 
  1000 & REAL\_OR\_ML & 1465.82 & 42.79 & 4950.00 &  &  &  &  \\ 
  1000 & SHRINKAGE & 1438.18 & 47.20 & 4950.00 &  &  &  & 0.04 \\ 
  1500 & GLASSO\_XVAL & 1427.13 & 12.36 & 2761.00 &  &  &  & 0.01 \\ 
  1500 & MFCF\_FIX & 867.20 & 35.90 & 1694.00 & 19.00 &  20 & 20.00 & 0.01 \\ 
  1500 & MFCF\_FIX\_ID & 867.38 & 35.82 & 1694.00 & 19.00 &  20 & 20.00 & 0.01 \\ 
  1500 & MFCF\_VAR & 815.21 & 42.09 & 1710.00 & 20.00 &  20 & 20.00 & 0.01 \\ 
  1500 & MFCF\_VAR\_ID & 815.28 & 42.04 & 1710.00 & 20.00 &  20 & 20.00 & 0.01 \\ 
  1500 & REAL\_OR\_ML & 1429.06 & 12.51 & 4950.00 &  &  &  &  \\ 
  1500 & SHRINKAGE & 1455.53 & 16.91 & 4950.00 &  &  &  & 0.04 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Performance of the models on a random clique forest. Mean values over 10 sample runs.} 
\label{tab:Factor:2}
\end{table}


==> Tables/Factor_paramno.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:09:58 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{|r|R{2cm}|R{2cm}|R{2cm}|R{2cm}|R{2cm}|R{2cm}|}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & SHRINKAGE \\ 
  \hline
25 & 1168 & 1694 & 1661 & 1582 & 1597 & 4950 \\ 
  50 & 1206 & 1677 & 1661 & 1694 & 1694 & 4950 \\ 
  75 & 1308 & 1661 & 1661 & 1678 & 1678 & 4950 \\ 
  100 & 1648 & 1710 & 1710 & 1645 & 1645 & 4950 \\ 
  200 & 2143 & 1710 & 1710 & 1678 & 1694 & 4950 \\ 
  300 & 2426 & 1710 & 1694 & 1694 & 1694 & 4950 \\ 
  400 & 2568 & 1710 & 1710 & 1710 & 1710 & 4950 \\ 
  500 & 2814 & 1694 & 1694 & 1694 & 1694 & 4950 \\ 
  750 & 2760 & 1694 & 1694 & 1694 & 1694 & 4950 \\ 
  1000 & 2755 & 1710 & 1710 & 1678 & 1678 & 4950 \\ 
  1500 & 2761 & 1694 & 1694 & 1710 & 1710 & 4950 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Mean number of non-zero coefficient in the precision matrix by length of time series} 
\label{tab:Factor:param_no}
\end{table}


==> Tables/Factor_shrink.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:09:57 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{|r|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & SHRINKAGE \\ 
  \hline
 25 & 0.12 & 0.27 & 0.26 & 0.25 & 0.25 & 0.30 \\ 
   50 & 0.12 & 0.19 & 0.18 & 0.18 & 0.18 & 0.23 \\ 
   75 & 0.09 & 0.15 & 0.14 & 0.15 & 0.15 & 0.20 \\ 
  100 & 0.06 & 0.13 & 0.13 & 0.12 & 0.12 & 0.18 \\ 
  200 & 0.02 & 0.08 & 0.08 & 0.08 & 0.08 & 0.14 \\ 
  300 & 0.01 & 0.06 & 0.06 & 0.06 & 0.06 & 0.11 \\ 
  400 & 0.01 & 0.05 & 0.05 & 0.05 & 0.05 & 0.09 \\ 
  500 & 0.01 & 0.04 & 0.04 & 0.04 & 0.04 & 0.08 \\ 
  750 & 0.01 & 0.03 & 0.03 & 0.03 & 0.03 & 0.06 \\ 
  1000 & 0.01 & 0.02 & 0.02 & 0.02 & 0.02 & 0.04 \\ 
  1500 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.04 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Mean penalty/shrinkage parameter by length of time series} 
\label{tab:Factor:shrink}
\end{table}


==> Tables/Factor_summary_ll.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:09:52 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rrrrrrrr}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & REAL\_OR\_ML & SHRINKAGE \\ 
  \hline
 25 & 61.12 & -313.06 & -279.57 & -341.81 & -334.90 & 1739.32 & 252.30 \\ 
   50 & 112.32 & 53.73 & 81.22 & 114.91 & 119.88 & 1614.94 & 552.55 \\ 
   75 & 450.13 & 233.31 & 265.18 & 265.91 & 268.30 & 1558.30 & 713.32 \\ 
  100 & 812.10 & 398.28 & 405.97 & 417.36 & 419.41 & 1523.66 & 789.05 \\ 
  200 & 1200.52 & 595.80 & 602.64 & 627.05 & 627.55 & 1497.52 & 1028.57 \\ 
  300 & 1334.60 & 759.23 & 764.49 & 696.99 & 697.17 & 1511.88 & 1190.94 \\ 
  400 & 1357.39 & 780.88 & 784.18 & 728.48 & 728.49 & 1489.11 & 1241.16 \\ 
  500 & 1350.93 & 757.01 & 758.04 & 755.60 & 755.42 & 1448.57 & 1265.29 \\ 
  750 & 1390.70 & 788.34 & 788.87 & 770.07 & 770.16 & 1434.73 & 1356.34 \\ 
  1000 & 1444.52 & 852.73 & 853.14 & 816.86 & 816.84 & 1465.82 & 1438.18 \\ 
  1500 & 1427.13 & 867.20 & 867.38 & 815.21 & 815.28 & 1429.06 & 1455.53 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Likelihood of the models. Mean values over 5 distinct training / validation sets and for 10 test set each.} 
\label{tab:Factor_summary:1}
\end{table}


==> Tables/Real.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:09:07 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rlrrrrrrr}
  \hline
Series length & Algorithm & Mean Log-likelihood & Stdev Log-likelihood & Mean number of parameters in inverse & Min clique size & Median clique size & Max clique size & Penalty/Shrinkage parameter \\ 
  \hline
 25 & GLASSO\_XVAL & -2463.20 & 561.75 & 950.00 &  &  &  & 0.21 \\ 
   25 & MFCF\_FIX & -2172.21 & 500.01 & 1561.00 & 14.00 &  19 & 20.00 & 0.81 \\ 
   25 & MFCF\_FIX\_ID & -2550.56 & 513.34 & 1478.00 & 13.00 &  18 & 19.00 & 0.57 \\ 
   25 & MFCF\_VAR & -2243.48 & 516.54 & 1206.00 & 11.00 &  16 & 20.00 & 0.80 \\ 
   25 & MFCF\_VAR\_ID & -2559.13 & 540.18 & 1055.00 & 11.00 &  11 & 17.00 & 0.54 \\ 
   25 & REAL\_OR\_ML & -1280.20 & 614.76 & 4950.00 &  &  &  &  \\ 
   25 & SHRINKAGE & -2558.49 & 547.64 & 4950.00 &  &  &  & 0.67 \\ 
   50 & GLASSO\_XVAL & -2528.49 & 467.24 & 1039.00 &  &  &  & 0.15 \\ 
   50 & MFCF\_FIX & -2427.37 & 414.08 & 1512.00 & 15.00 &  18 & 20.00 & 0.73 \\ 
   50 & MFCF\_FIX\_ID & -2670.42 & 456.89 & 1010.00 & 6.00 &  14 & 15.00 & 0.47 \\ 
   50 & MFCF\_VAR & -2438.69 & 424.69 & 1286.00 & 11.00 &  16 & 18.00 & 0.70 \\ 
   50 & MFCF\_VAR\_ID & -2674.56 & 450.48 & 1018.00 & 7.00 &  10 & 18.00 & 0.47 \\ 
   50 & REAL\_OR\_ML & -1461.33 & 377.11 & 4950.00 &  &  &  &  \\ 
   50 & SHRINKAGE & -2725.01 & 403.24 & 4950.00 &  &  &  & 0.63 \\ 
   75 & GLASSO\_XVAL & -2618.80 & 376.90 & 1099.00 &  &  &  & 0.12 \\ 
   75 & MFCF\_FIX & -2621.05 & 376.88 & 1628.00 & 17.00 &  19 & 20.00 & 0.62 \\ 
   75 & MFCF\_FIX\_ID & -2761.78 & 377.99 & 798.00 & 7.00 &  10 & 13.00 & 0.35 \\ 
   75 & MFCF\_VAR & -2619.53 & 378.59 & 1416.00 & 14.00 &  16 & 20.00 & 0.61 \\ 
   75 & MFCF\_VAR\_ID & -2759.37 & 386.19 & 850.00 & 8.00 &  10 & 11.00 & 0.36 \\ 
   75 & REAL\_OR\_ML & -1836.75 & 341.94 & 4950.00 &  &  &  &  \\ 
   75 & SHRINKAGE & -2821.22 & 323.63 & 4950.00 &  &  &  & 0.55 \\ 
  100 & GLASSO\_XVAL & -2610.36 & 263.15 & 1063.00 &  &  &  & 0.12 \\ 
  100 & MFCF\_FIX & -2578.57 & 244.60 & 1545.00 & 15.00 &  18 & 20.00 & 0.56 \\ 
  100 & MFCF\_FIX\_ID & -2684.32 & 274.86 & 1053.00 & 5.00 &  15 & 19.00 & 0.31 \\ 
  100 & MFCF\_VAR & -2572.94 & 250.00 & 1310.00 & 11.00 &  16 & 17.00 & 0.54 \\ 
  100 & MFCF\_VAR\_ID & -2699.43 & 276.30 & 1060.00 & 5.00 &  13 & 17.00 & 0.33 \\ 
  100 & REAL\_OR\_ML & -1822.45 & 226.94 & 4950.00 &  &  &  &  \\ 
  100 & SHRINKAGE & -2799.69 & 234.66 & 4950.00 &  &  &  & 0.54 \\ 
  200 & GLASSO\_XVAL & -2605.54 & 176.13 & 1057.00 &  &  &  & 0.12 \\ 
  200 & MFCF\_FIX & -2495.72 & 191.90 & 1363.00 & 15.00 &  16 & 17.00 & 0.43 \\ 
  200 & MFCF\_FIX\_ID & -2555.83 & 183.12 & 1152.00 & 9.00 &  15 & 17.00 & 0.26 \\ 
  200 & MFCF\_VAR & -2506.77 & 186.58 & 1443.00 & 12.00 &  18 & 20.00 & 0.44 \\ 
  200 & MFCF\_VAR\_ID & -2561.94 & 191.19 & 1094.00 & 6.00 &  13 & 19.00 & 0.26 \\ 
  200 & REAL\_OR\_ML & -1958.70 & 203.50 & 4950.00 &  &  &  &  \\ 
  200 & SHRINKAGE & -2664.73 & 173.99 & 4950.00 &  &  &  & 0.44 \\ 
  300 & GLASSO\_XVAL & -2613.91 & 165.49 & 1170.00 &  &  &  & 0.10 \\ 
  300 & MFCF\_FIX & -2527.65 & 110.87 & 1202.00 & 9.00 &  14 & 20.00 & 0.32 \\ 
  300 & MFCF\_FIX\_ID & -2556.48 & 117.19 & 1049.00 & 9.00 &  12 & 15.00 & 0.20 \\ 
  300 & MFCF\_VAR & -2524.18 & 109.91 & 1375.00 & 11.00 &  18 & 19.00 & 0.34 \\ 
  300 & MFCF\_VAR\_ID & -2553.71 & 116.45 & 888.00 & 7.00 &   9 & 14.00 & 0.18 \\ 
  300 & REAL\_OR\_ML & -2089.36 & 124.46 & 4950.00 &  &  &  &  \\ 
  300 & SHRINKAGE & -2662.54 & 91.80 & 4950.00 &  &  &  & 0.39 \\ 
  400 & GLASSO\_XVAL & -2618.82 & 115.02 & 1191.00 &  &  &  & 0.08 \\ 
  400 & MFCF\_FIX & -2606.22 & 127.00 & 1359.00 & 11.00 &  16 & 19.00 & 0.28 \\ 
  400 & MFCF\_FIX\_ID & -2628.84 & 132.69 & 1154.00 & 10.00 &  15 & 16.00 & 0.17 \\ 
  400 & MFCF\_VAR & -2607.56 & 128.36 & 1325.00 & 10.00 &  16 & 19.00 & 0.28 \\ 
  400 & MFCF\_VAR\_ID & -2630.98 & 135.44 & 1255.00 & 10.00 &  15 & 19.00 & 0.17 \\ 
  400 & REAL\_OR\_ML & -2185.06 & 121.92 & 4950.00 &  &  &  &  \\ 
  400 & SHRINKAGE & -2705.29 & 123.78 & 4950.00 &  &  &  & 0.34 \\ 
  500 & GLASSO\_XVAL & -2583.27 & 118.14 & 1464.00 &  &  &  & 0.07 \\ 
  500 & MFCF\_FIX & -2551.57 & 101.05 & 1578.00 & 15.00 &  19 & 20.00 & 0.25 \\ 
  500 & MFCF\_FIX\_ID & -2571.16 & 104.75 & 1358.00 & 11.00 &  15 & 20.00 & 0.15 \\ 
  500 & MFCF\_VAR & -2554.57 & 107.02 & 1477.00 & 13.00 &  18 & 20.00 & 0.24 \\ 
  500 & MFCF\_VAR\_ID & -2572.88 & 108.73 & 1360.00 & 13.00 &  15 & 20.00 & 0.15 \\ 
  500 & REAL\_OR\_ML & -2171.48 & 90.89 & 4950.00 &  &  &  &  \\ 
  500 & SHRINKAGE & -2628.21 & 100.11 & 4950.00 &  &  &  & 0.30 \\ 
  750 & GLASSO\_XVAL & -2450.17 & 133.47 & 1994.00 &  &  &  & 0.03 \\ 
  750 & MFCF\_FIX & -2521.73 & 127.98 & 1495.00 & 14.00 &  17 & 20.00 & 0.18 \\ 
  750 & MFCF\_FIX\_ID & -2531.22 & 127.91 & 1495.00 & 14.00 &  17 & 20.00 & 0.12 \\ 
  750 & MFCF\_VAR & -2516.58 & 119.49 & 1562.00 & 16.00 &  18 & 20.00 & 0.19 \\ 
  750 & MFCF\_VAR\_ID & -2527.05 & 118.97 & 1562.00 & 16.00 &  18 & 20.00 & 0.13 \\ 
  750 & REAL\_OR\_ML & -2205.35 & 136.63 & 4950.00 &  &  &  &  \\ 
  750 & SHRINKAGE & -2563.06 & 133.81 & 4950.00 &  &  &  & 0.24 \\ 
  1000 & GLASSO\_XVAL & -2493.24 & 75.05 & 2404.00 &  &  &  & 0.02 \\ 
  1000 & MFCF\_FIX & -2563.27 & 81.04 & 1595.00 & 15.00 &  19 & 20.00 & 0.13 \\ 
  1000 & MFCF\_FIX\_ID & -2569.82 & 82.61 & 1595.00 & 15.00 &  19 & 20.00 & 0.08 \\ 
  1000 & MFCF\_VAR & -2563.31 & 80.59 & 1645.00 & 17.00 &  20 & 20.00 & 0.13 \\ 
  1000 & MFCF\_VAR\_ID & -2569.77 & 82.74 & 1645.00 & 17.00 &  20 & 20.00 & 0.08 \\ 
  1000 & REAL\_OR\_ML & -2311.93 & 69.38 & 4950.00 &  &  &  &  \\ 
  1000 & SHRINKAGE & -2568.76 & 79.71 & 4950.00 &  &  &  & 0.17 \\ 
  1500 & GLASSO\_XVAL & -2467.06 & 71.83 & 2752.00 &  &  &  & 0.01 \\ 
  1500 & MFCF\_FIX & -2549.02 & 62.65 & 1710.00 & 20.00 &  20 & 20.00 & 0.11 \\ 
  1500 & MFCF\_FIX\_ID & -2553.15 & 61.77 & 1677.00 & 18.00 &  20 & 20.00 & 0.07 \\ 
  1500 & MFCF\_VAR & -2552.45 & 63.82 & 1645.00 & 18.00 &  19 & 20.00 & 0.11 \\ 
  1500 & MFCF\_VAR\_ID & -2556.22 & 62.97 & 1629.00 & 18.00 &  19 & 20.00 & 0.07 \\ 
  1500 & REAL\_OR\_ML & -2340.61 & 72.24 & 4950.00 &  &  &  &  \\ 
  1500 & SHRINKAGE & -2519.63 & 65.35 & 4950.00 &  &  &  & 0.14 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Likelihood of the models. Mean values over 5 distinct training / validation sets and for 10 test set each.} 
\label{tab:Real:1}
\end{table}


==> Tables/Real_acc.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:09:07 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rlrrrrrrr}
  \hline
Series length & Algorithm & Mean Log-likelihood & Stdev Log-likelihood & Mean number of parameters in inverse & Min clique size & Median clique size & Max clique size & Penalty/Shrinkage parameter \\ 
  \hline
 25 & GLASSO\_XVAL & -2463.20 & 561.75 & 950.00 &  &  &  & 0.21 \\ 
   25 & MFCF\_FIX & -2172.21 & 500.01 & 1561.00 & 14.00 &  19 & 20.00 & 0.81 \\ 
   25 & MFCF\_FIX\_ID & -2550.56 & 513.34 & 1478.00 & 13.00 &  18 & 19.00 & 0.57 \\ 
   25 & MFCF\_VAR & -2243.48 & 516.54 & 1206.00 & 11.00 &  16 & 20.00 & 0.80 \\ 
   25 & MFCF\_VAR\_ID & -2559.13 & 540.18 & 1055.00 & 11.00 &  11 & 17.00 & 0.54 \\ 
   25 & REAL\_OR\_ML & -1280.20 & 614.76 & 4950.00 &  &  &  &  \\ 
   25 & SHRINKAGE & -2558.49 & 547.64 & 4950.00 &  &  &  & 0.67 \\ 
   50 & GLASSO\_XVAL & -2528.49 & 467.24 & 1039.00 &  &  &  & 0.15 \\ 
   50 & MFCF\_FIX & -2427.37 & 414.08 & 1512.00 & 15.00 &  18 & 20.00 & 0.73 \\ 
   50 & MFCF\_FIX\_ID & -2670.42 & 456.89 & 1010.00 & 6.00 &  14 & 15.00 & 0.47 \\ 
   50 & MFCF\_VAR & -2438.69 & 424.69 & 1286.00 & 11.00 &  16 & 18.00 & 0.70 \\ 
   50 & MFCF\_VAR\_ID & -2674.56 & 450.48 & 1018.00 & 7.00 &  10 & 18.00 & 0.47 \\ 
   50 & REAL\_OR\_ML & -1461.33 & 377.11 & 4950.00 &  &  &  &  \\ 
   50 & SHRINKAGE & -2725.01 & 403.24 & 4950.00 &  &  &  & 0.63 \\ 
   75 & GLASSO\_XVAL & -2618.80 & 376.90 & 1099.00 &  &  &  & 0.12 \\ 
   75 & MFCF\_FIX & -2621.05 & 376.88 & 1628.00 & 17.00 &  19 & 20.00 & 0.62 \\ 
   75 & MFCF\_FIX\_ID & -2761.78 & 377.99 & 798.00 & 7.00 &  10 & 13.00 & 0.35 \\ 
   75 & MFCF\_VAR & -2619.53 & 378.59 & 1416.00 & 14.00 &  16 & 20.00 & 0.61 \\ 
   75 & MFCF\_VAR\_ID & -2759.37 & 386.19 & 850.00 & 8.00 &  10 & 11.00 & 0.36 \\ 
   75 & REAL\_OR\_ML & -1836.75 & 341.94 & 4950.00 &  &  &  &  \\ 
   75 & SHRINKAGE & -2821.22 & 323.63 & 4950.00 &  &  &  & 0.55 \\ 
  100 & GLASSO\_XVAL & -2610.36 & 263.15 & 1063.00 &  &  &  & 0.12 \\ 
  100 & MFCF\_FIX & -2578.57 & 244.60 & 1545.00 & 15.00 &  18 & 20.00 & 0.56 \\ 
  100 & MFCF\_FIX\_ID & -2684.32 & 274.86 & 1053.00 & 5.00 &  15 & 19.00 & 0.31 \\ 
  100 & MFCF\_VAR & -2572.94 & 250.00 & 1310.00 & 11.00 &  16 & 17.00 & 0.54 \\ 
  100 & MFCF\_VAR\_ID & -2699.43 & 276.30 & 1060.00 & 5.00 &  13 & 17.00 & 0.33 \\ 
  100 & REAL\_OR\_ML & -1822.45 & 226.94 & 4950.00 &  &  &  &  \\ 
  100 & SHRINKAGE & -2799.69 & 234.66 & 4950.00 &  &  &  & 0.54 \\ 
  200 & GLASSO\_XVAL & -2605.54 & 176.13 & 1057.00 &  &  &  & 0.12 \\ 
  200 & MFCF\_FIX & -2495.72 & 191.90 & 1363.00 & 15.00 &  16 & 17.00 & 0.43 \\ 
  200 & MFCF\_FIX\_ID & -2555.83 & 183.12 & 1152.00 & 9.00 &  15 & 17.00 & 0.26 \\ 
  200 & MFCF\_VAR & -2506.77 & 186.58 & 1443.00 & 12.00 &  18 & 20.00 & 0.44 \\ 
  200 & MFCF\_VAR\_ID & -2561.94 & 191.19 & 1094.00 & 6.00 &  13 & 19.00 & 0.26 \\ 
  200 & REAL\_OR\_ML & -1958.70 & 203.50 & 4950.00 &  &  &  &  \\ 
  200 & SHRINKAGE & -2664.73 & 173.99 & 4950.00 &  &  &  & 0.44 \\ 
  300 & GLASSO\_XVAL & -2613.91 & 165.49 & 1170.00 &  &  &  & 0.10 \\ 
  300 & MFCF\_FIX & -2527.65 & 110.87 & 1202.00 & 9.00 &  14 & 20.00 & 0.32 \\ 
  300 & MFCF\_FIX\_ID & -2556.48 & 117.19 & 1049.00 & 9.00 &  12 & 15.00 & 0.20 \\ 
  300 & MFCF\_VAR & -2524.18 & 109.91 & 1375.00 & 11.00 &  18 & 19.00 & 0.34 \\ 
  300 & MFCF\_VAR\_ID & -2553.71 & 116.45 & 888.00 & 7.00 &   9 & 14.00 & 0.18 \\ 
  300 & REAL\_OR\_ML & -2089.36 & 124.46 & 4950.00 &  &  &  &  \\ 
  300 & SHRINKAGE & -2662.54 & 91.80 & 4950.00 &  &  &  & 0.39 \\ 
  400 & GLASSO\_XVAL & -2618.82 & 115.02 & 1191.00 &  &  &  & 0.08 \\ 
  400 & MFCF\_FIX & -2606.22 & 127.00 & 1359.00 & 11.00 &  16 & 19.00 & 0.28 \\ 
  400 & MFCF\_FIX\_ID & -2628.84 & 132.69 & 1154.00 & 10.00 &  15 & 16.00 & 0.17 \\ 
  400 & MFCF\_VAR & -2607.56 & 128.36 & 1325.00 & 10.00 &  16 & 19.00 & 0.28 \\ 
  400 & MFCF\_VAR\_ID & -2630.98 & 135.44 & 1255.00 & 10.00 &  15 & 19.00 & 0.17 \\ 
  400 & REAL\_OR\_ML & -2185.06 & 121.92 & 4950.00 &  &  &  &  \\ 
  400 & SHRINKAGE & -2705.29 & 123.78 & 4950.00 &  &  &  & 0.34 \\ 
  500 & GLASSO\_XVAL & -2583.27 & 118.14 & 1464.00 &  &  &  & 0.07 \\ 
  500 & MFCF\_FIX & -2551.57 & 101.05 & 1578.00 & 15.00 &  19 & 20.00 & 0.25 \\ 
  500 & MFCF\_FIX\_ID & -2571.16 & 104.75 & 1358.00 & 11.00 &  15 & 20.00 & 0.15 \\ 
  500 & MFCF\_VAR & -2554.57 & 107.02 & 1477.00 & 13.00 &  18 & 20.00 & 0.24 \\ 
  500 & MFCF\_VAR\_ID & -2572.88 & 108.73 & 1360.00 & 13.00 &  15 & 20.00 & 0.15 \\ 
  500 & REAL\_OR\_ML & -2171.48 & 90.89 & 4950.00 &  &  &  &  \\ 
  500 & SHRINKAGE & -2628.21 & 100.11 & 4950.00 &  &  &  & 0.30 \\ 
  750 & GLASSO\_XVAL & -2450.17 & 133.47 & 1994.00 &  &  &  & 0.03 \\ 
  750 & MFCF\_FIX & -2521.73 & 127.98 & 1495.00 & 14.00 &  17 & 20.00 & 0.18 \\ 
  750 & MFCF\_FIX\_ID & -2531.22 & 127.91 & 1495.00 & 14.00 &  17 & 20.00 & 0.12 \\ 
  750 & MFCF\_VAR & -2516.58 & 119.49 & 1562.00 & 16.00 &  18 & 20.00 & 0.19 \\ 
  750 & MFCF\_VAR\_ID & -2527.05 & 118.97 & 1562.00 & 16.00 &  18 & 20.00 & 0.13 \\ 
  750 & REAL\_OR\_ML & -2205.35 & 136.63 & 4950.00 &  &  &  &  \\ 
  750 & SHRINKAGE & -2563.06 & 133.81 & 4950.00 &  &  &  & 0.24 \\ 
  1000 & GLASSO\_XVAL & -2493.24 & 75.05 & 2404.00 &  &  &  & 0.02 \\ 
  1000 & MFCF\_FIX & -2563.27 & 81.04 & 1595.00 & 15.00 &  19 & 20.00 & 0.13 \\ 
  1000 & MFCF\_FIX\_ID & -2569.82 & 82.61 & 1595.00 & 15.00 &  19 & 20.00 & 0.08 \\ 
  1000 & MFCF\_VAR & -2563.31 & 80.59 & 1645.00 & 17.00 &  20 & 20.00 & 0.13 \\ 
  1000 & MFCF\_VAR\_ID & -2569.77 & 82.74 & 1645.00 & 17.00 &  20 & 20.00 & 0.08 \\ 
  1000 & REAL\_OR\_ML & -2311.93 & 69.38 & 4950.00 &  &  &  &  \\ 
  1000 & SHRINKAGE & -2568.76 & 79.71 & 4950.00 &  &  &  & 0.17 \\ 
  1500 & GLASSO\_XVAL & -2467.06 & 71.83 & 2752.00 &  &  &  & 0.01 \\ 
  1500 & MFCF\_FIX & -2549.02 & 62.65 & 1710.00 & 20.00 &  20 & 20.00 & 0.11 \\ 
  1500 & MFCF\_FIX\_ID & -2553.15 & 61.77 & 1677.00 & 18.00 &  20 & 20.00 & 0.07 \\ 
  1500 & MFCF\_VAR & -2552.45 & 63.82 & 1645.00 & 18.00 &  19 & 20.00 & 0.11 \\ 
  1500 & MFCF\_VAR\_ID & -2556.22 & 62.97 & 1629.00 & 18.00 &  19 & 20.00 & 0.07 \\ 
  1500 & REAL\_OR\_ML & -2340.61 & 72.24 & 4950.00 &  &  &  &  \\ 
  1500 & SHRINKAGE & -2519.63 & 65.35 & 4950.00 &  &  &  & 0.14 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Performance of the models on a random clique forest. Mean values over 10 sample runs.} 
\label{tab:Real:2}
\end{table}


==> Tables/Real_paramno.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:09:14 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{|r|R{2cm}|R{2cm}|R{2cm}|R{2cm}|R{2cm}|R{2cm}|}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & SHRINKAGE \\ 
  \hline
25 & 950 & 1561 & 1478 & 1206 & 1055 & 4950 \\ 
  50 & 1039 & 1512 & 1010 & 1286 & 1018 & 4950 \\ 
  75 & 1099 & 1628 & 798 & 1416 & 850 & 4950 \\ 
  100 & 1063 & 1545 & 1053 & 1310 & 1060 & 4950 \\ 
  200 & 1057 & 1363 & 1152 & 1443 & 1094 & 4950 \\ 
  300 & 1170 & 1202 & 1049 & 1375 & 888 & 4950 \\ 
  400 & 1191 & 1359 & 1154 & 1325 & 1255 & 4950 \\ 
  500 & 1464 & 1578 & 1358 & 1477 & 1360 & 4950 \\ 
  750 & 1994 & 1495 & 1495 & 1562 & 1562 & 4950 \\ 
  1000 & 2404 & 1595 & 1595 & 1645 & 1645 & 4950 \\ 
  1500 & 2752 & 1710 & 1677 & 1645 & 1629 & 4950 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Mean number of non-zero coefficient in the precision matrix by length of time series} 
\label{tab:Real:param_no}
\end{table}


==> Tables/Real_shrink.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:09:14 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{|r|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|C{2cm}|}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & SHRINKAGE \\ 
  \hline
  25 & 0.208 & 0.814 & 0.566 & 0.799 & 0.544 & 0.669 \\ 
    50 & 0.149 & 0.730 & 0.469 & 0.702 & 0.471 & 0.627 \\ 
    75 & 0.121 & 0.624 & 0.355 & 0.615 & 0.364 & 0.552 \\ 
   100 & 0.125 & 0.565 & 0.310 & 0.545 & 0.327 & 0.540 \\ 
   200 & 0.120 & 0.430 & 0.263 & 0.440 & 0.255 & 0.444 \\ 
   300 & 0.103 & 0.316 & 0.196 & 0.335 & 0.179 & 0.386 \\ 
   400 & 0.081 & 0.285 & 0.168 & 0.281 & 0.175 & 0.344 \\ 
   500 & 0.069 & 0.248 & 0.148 & 0.238 & 0.147 & 0.300 \\ 
   750 & 0.028 & 0.184 & 0.120 & 0.192 & 0.126 & 0.242 \\ 
  1000 & 0.020 & 0.127 & 0.081 & 0.127 & 0.082 & 0.172 \\ 
  1500 & 0.013 & 0.113 & 0.073 & 0.111 & 0.072 & 0.141 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Mean penalty/shrinkage parameter by length of time series} 
\label{tab:Real:shrink}
\end{table}


==> Tables/Real_summary_ll.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu May 13 15:09:07 2021
\begin{table}[ht]
\centering
\begingroup\footnotesize
\begin{tabular}{rrrrrrrr}
  \hline
Series length & GLASSO\_XVAL & MFCF\_FIX & MFCF\_FIX\_ID & MFCF\_VAR & MFCF\_VAR\_ID & REAL\_OR\_ML & SHRINKAGE \\ 
  \hline
 25 & -2463.20 & -2172.21 & -2550.56 & -2243.48 & -2559.13 & -1280.20 & -2558.49 \\ 
   50 & -2528.49 & -2427.37 & -2670.42 & -2438.69 & -2674.56 & -1461.33 & -2725.01 \\ 
   75 & -2618.80 & -2621.05 & -2761.78 & -2619.53 & -2759.37 & -1836.75 & -2821.22 \\ 
  100 & -2610.36 & -2578.57 & -2684.32 & -2572.94 & -2699.43 & -1822.45 & -2799.69 \\ 
  200 & -2605.54 & -2495.72 & -2555.83 & -2506.77 & -2561.94 & -1958.70 & -2664.73 \\ 
  300 & -2613.91 & -2527.65 & -2556.48 & -2524.18 & -2553.71 & -2089.36 & -2662.54 \\ 
  400 & -2618.82 & -2606.22 & -2628.84 & -2607.56 & -2630.98 & -2185.06 & -2705.29 \\ 
  500 & -2583.27 & -2551.57 & -2571.16 & -2554.57 & -2572.88 & -2171.48 & -2628.21 \\ 
  750 & -2450.17 & -2521.73 & -2531.22 & -2516.58 & -2527.05 & -2205.35 & -2563.06 \\ 
  1000 & -2493.24 & -2563.27 & -2569.82 & -2563.31 & -2569.77 & -2311.93 & -2568.76 \\ 
  1500 & -2467.06 & -2549.02 & -2553.15 & -2552.45 & -2556.22 & -2340.61 & -2519.63 \\ 
   \hline
\end{tabular}
\endgroup
\caption{Likelihood of the models. Mean values over 5 distinct training / validation sets and for 10 test set each.} 
\label{tab:Real_summary:1}
\end{table}

